Bug Hunters' Perspectives on the Challenges and Benefits of the Bug Bounty Ecosystem

Although researchers have characterized the bug-bounty ecosystem from the point of view of platforms and programs, minimal effort has been made to understand the perspectives of the main workers: bug hunters. To improve bug bounties, it is important to understand hunters' motivating factors, challenges, and overall benefits. We address this research gap with three studies: identifying key factors through a free listing survey (n=56), rating each factor's importance with a larger-scale factor-rating survey (n=159), and conducting semi-structured interviews to uncover details (n=24). Of 54 factors that bug hunters listed, we find that rewards and learning opportunities are the most important benefits. Further, we find scope to be the top differentiator between programs. Surprisingly, we find earning reputation to be one of the least important motivators for hunters. Of the challenges we identify, communication problems, such as unresponsiveness and disputes, are the most substantial. We present recommendations to make the bug-bounty ecosystem accommodating to more bug hunters and ultimately increase participation in an underutilized market.

==> statement.tex <==
\onecolumn
\pagestyle{plain}
\setlength{\parskip}{\baselineskip}
\setlength{\parindent}{0pt}

\newcounter{reviewercomment}[section]
\newcommand{\reviewerComment}[2]{\refstepcounter{reviewercomment} \textbf{Criterion~\thereviewercomment:} \textit{``#2''}}
\definecolor{darkblue}{rgb}{0,0,0.5}
\newcommand{\response}[1]{\underline{Changes:} {#1} \vspace{0.1in}}
\newcommand{\paperQuote}[1]{\color{darkblue}``\textit{#1}''\color{black}}

\begin{center}
\Large{Summary of Changes}\\
\vspace{0.1in}
\large{\textbf{Bug Hunters' Perspectives on the Challenges and Benefits of  the Bug Bounty Ecosystem}}\\
\vspace{0.075in}
{Major Revision (USENIX Security'22 Winter)}
\end{center}

We again thank the reviewers for their thoughtful comments. Please find a summary of how we addressed issues that were brought up below. We also include a ``diff'' of the previous submission and the revised version. Due to the large number of edits, the ``diff'' can look convoluted. Red highlights show deleted segments from the old version to the new version, and green highlights show additions in the new version.

\reviewerComment{}{For factors in Table 2, more thoroughly compare with prior research that also discussed similar types of factors and explicitly explain which factors were newly discovered and which have been covered by prior research.}

\response{We have made the following major changes:
\begin{itemize}[noitemsep,topsep=0pt]
    \item Added citations for work that found factors that we also identify in Table~\ref{tab:refined_codes}.
    \item Explained how our work differs in the Introduction (page 2), Related work (``Hunters’ self-reported motivation''), and Factors (first paragraph) sections. 
\end{itemize}
}

We argue in Section~\ref{sec:intro} (Introduction):

\paperQuote{\Bbplatforms have themselves issued several reports on \hunters' motivations~\cite{bugcrowd2021report, bugcrowd2020report, bugcrowd2018report, hackerone2019report,hackerone2020report,hackerone2021report}. However, 
these brief reports do not focus on challenges faced by \hunters, appear to be for marketing, and are not independently verified. }

\paperQuote{Other research efforts have used interviews with stakeholders throughout vulnerability disclosure, including bug bounty programs, to explore drawbacks of the gig-work model~\cite{ellis2022bounty} and challenges in the vulnerability discovery ecosystem as a whole~\cite{alomar2020nicebugs}. We build upon these broad, qualitative studies with a larger, mixed-methods sample that explicitly and systematically identifies and quantifies the factors that affect \hunters' participation in \bbprograms. Unlike prior work, we ask \hunters to quantify how important individual factors are, allowing stakeholders to know which factors to prioritize. For instance, like other researchers~\cite{ellis2022bounty,walshe2020empirical}, we find reputation to be a motivator; however, we are able to demonstrate that it is in fact one of the least important motivators (\autoref{sec:rewards}).}

In Section~\ref{sec:factors} (Factors), we further clarify specific contribution differences:

\paperQuote{We identified 54 factors affecting participation in the \bb ecosystem under four \hlqs. A complete list can be found in~\autoref{tab:refined_codes}.
Some of these factors are reported in prior work; 
as shown in \autoref{tab:refined_codes}, no previous work 
has systematically identified all factors, and most focus on 
benefits, leaving gaps in challenges and in which 
platform features are most useful. Further, we provide the first 
in-depth ranking of factor importance. }





\reviewerComment{}{For the factor-ranking study, please analyze the rank data and report the results following well-established guidelines of statistical analysis methods, e.g., Alvo, Mayer, and L. H. Philip. Statistical methods for ranking data. Vol. 1341. New York: Springer, 2014. Note that this paper is just an example of methodology paper. If the authors choose methods recommended by other sources please also cite them in your paper.}

\response{We have used LLBT-based modeling to reason about the importance of factors. We explain the rationale and how to interpret these numbers in Section~\ref{subsec:ratingmethods}:

\paperQuote{A straightforward (and common) 
way of analyzing which factors are the most important would be to convert our participants' Likert choices to numeric values and present simple averages. This approach, while seemingly intuitive, has been criticized and discouraged by statisticians~\cite{dittrich2007paired,lubke2004applying,wu2007empirical}, because it makes the dubious assumption that the ordinal options that participants select are equidistant (e.g., the distance between ``Extremely important'' and ``Very important'' is the same as between ``Very important'' and ``Moderately important''). Thus, we adopt comparison-based techniques, which consider only whether one factor is rated higher than another. Specifically, we employ log-linear Bradley-Terry (LLBT) modeling to synthesize \emph{worth} estimates ($\pi$) that represent the relative importance of factors ($f$) to participants on a preference scale~\cite{dittrich1998modelling, dittrich2007paired}. The probability of one factor being preferred over another is given by: 
\setlength{\abovedisplayskip}{4pt}
\[p(f_j>f_k|\pi_j,\pi_j)=\frac{\pi_j}{\pi_j+\pi_k}\]
\setlength{\belowdisplayskip}{0pt}
where $j,k$ denote the indices of factors considered~\cite{dittrich2009fitting}.}

\paperQuote{We use a version of LLBT
that requires converting our data to explicit paired comparisons. Methods without this conversion are computationally infeasible for our high-dimensional data~\cite{dittrich2007paired, hatzinger2012prefmod}. Researchers who developed these statistical methods confirmed that our approach is appropriate~\cite{akgul2022privatecomm}.
}

We have updated the relevant numbers throughout Section~\ref{sec:factors} and Table~\ref{tab:refined_codes} (last column). We have made minor changes in the text (Section~\ref{sec:factors}) to reflect the minor result changes from the previous analysis to the new one.
}

\reviewerComment{}{Please remove RQ3 and Section 6.1. This section as-is doesn't provide conclusive, meaningful insights. Removing this section won't hurt the main contribution and it will also leave space for extending the discussions.}

\response{We have removed Section 6. We have also removed the relevant parts of the introduction and the discussion of methods.}

\reviewerComment{}{Acknowledge and quantify selection bias and explore its implications for the findings.}


\reviewerComment{}{Acknowledge potential validity issues in the survey and reflect on their scope and impact.}

\response{We have made the following major changes to address the two criteria above:
\begin{itemize}[noitemsep, topsep=0pt]
    \item We have added the entries after “Education” in Table~\ref{tab:demo} to show the breadth of our participants' skills, experience, and working arrangements.
    \item We have expanded the discussion in Sections~\ref{sec:limitations} and~\ref{sec:demographics}
    to acknowledge and address demographic and selection biases. We compare our sample to samples from a bug-bounty platforms report in the text in Section ~\ref{sec:demographics}. While our sample is less educated, it generally mirrors samples reported by large \bbplatforms in other respects. Further, our participants report a wide range of experience and skill levels. Note, we did not include a comparison of \hunters who did or did not respond to our direct emails, as requested by RD. We did not precisely keep track of which avenues our participants were recruited (this is why we can only give rough estimates in the paper, see ``Recruitment'' in Section~\ref{subsec:ratingmethods}), meaning it would be impossible for us to determine whether this was or was not a direct contact, unpredictably skewing any result we might report. Instead, we compare to \hunter demographics from other surveys to demonstrate the similarity of our populations to \hunters recruited using other means.
    \item We clarified that pilots did result in changes to the procedures intended to reduce validity issues (Section~\ref{sec:limitations}). 
\end{itemize}}

\paperQuote{\Hunters might have portrayed themselves as more successful than they are. Similarly, our gift card incentive might have been most attractive to interview participants who make less money in \bbprograms, perhaps due to lower skill or experience. We partially addressed this by recruiting the majority of \firststudyps from non-public \hunter messaging channels and \secondstudyps from \hunters from authors of publicly disclosed bugs, implying some level of expertise. Further, the metrics we collected indicate a relatively even distribution across all skill and experience levels (see~\autoref{tab:demo}).}

\paperQuote{On the other hand, it is likely we did not capture people who wanted to participate in \bbs but were unable to at all. This problem of survivor bias is likely unavoidable, as there is no clear way to recruit people interested, but not active in \bbs. However, we expect some of our participants with less \bb participation will have similar experiences.}

\paperQuote{Further, all three of our studies, like all self-report studies~\cite{breen2022large}, include some sampling and selection biases. Our sample is likely reasonably representative of the current \hacker population (\autoref{sec:demographics}) and includes diversity in participant location, education, experience, and skill, meaning our results are reasonably likely to generalize to the average \hunter. However, the \hunter population itself is demographically skewed (e.g., young, white or Southeast Asian, and male~\cite{hackerone2020report,bugcrowd2020report, bugcrowd2021report}), likely introducing inherent biases 
(e.g., the companies and vulnerabilities that get attention). 
For a discussion of marginalized populations, we refer readers to the work of Fulton et al.~\cite{fulton2023v4a}.}

\reviewerComment{}{Improved framing of the problem, explaining how quantification adds insights to what we already know, as discussed by Review D and in the rebuttal.}

\response{We changed the introduction, and discussion sections to explain that quantification allows for determination of the most pressing issues and most valuable features/benefits. We recommend supporting/addressing these factors for the most efficient improvements in \bbs.

We give examples throughout the text to show how our results support or contradict factors that other researchers found to be important.


For instance, we note:
}

\paperQuote{Though 14 \firststudyps mentioned reputation as an overall benefit, \secondstudyps gave it limited importance, rating it the second least important benefit ({\w0.048}). Similarly, the \emph{reputation systems} that \bbplatforms provide were rated the second least important feature (\FL{6}, \w{5}). We speculate that although reputation is a very visible aspect of bug bounties, 
it's ultimately not as beneficial as other factors. This finding contradicts prior work that hypothesizes 
reputation might be more important than or comparable to monetary compensation~\cite{ellis2018empbounty, walshe2020empirical, sridhar2021hacking}.}


The discussion section prioritizes factors we found to be important to hunters to give better guidance in light of our results. For instance, we suggest:

\paperQuote{Beyond improving less popular aspects, \bbplatforms should not neglect their most popular features: providing a wide range of payment mechanisms (e.g., for international \hunters), standardizing interfaces between programs, and enabling \hunters to review (and read others' reviews of) \bbprograms.}



\reviewerComment{}{In the discussion, reflect on some of the societal, technical, and legal implications of these findings (see Review C).}

\response{We have reframed the paper to discuss the underutilization of bug bounty programs, and unequal benefit distribution of the ecosystem (paragraph 4 in Section~\ref{sec:intro}).
 
We argue that by reducing challenges of bug bounties and supporting benefits/useful features, bug bounties can improve the security of more companies and benefit more hunters.  In the discussion we note:}




\paperQuote{When the ecosystem functions well, \bbs have the potential to improve the security posture of organizations (commercial or governmental) at a low cost~\cite{sridhar2021hacking, walshe2020empirical}, while also providing \hunters numerous benefits. However, \bbs have low adoption rates, and only some organizations that run \bbs consistently attract quality bug reports~\cite{maillart2017given, sridhar2021hacking}. On the \hunters' side, while the reported pool of workers is large, only a few receive the full breadth of promised benefits~\cite{ellis2022bounty}. Essentially, not only are \bbs underutilized, but there exist inequalities in how the current ecosystem's benefits are distributed among organizations and \hunters.}

\paperQuote{In this section, we list recommendations for \bbprograms, platforms, and policymakers to alleviate the important challenges we have identified, as well as support and expand the benefits \hunters appreciate the most. We hope this can bolster \bb adoption, helping the security of more organizations, and ensuring more \hunters receive the full benefits of this marketplace.}


We have further acknowledged demographic skews and pointed to relevant work in Section~\ref{sec:limitations}. We have added a discussion section on what role governments might play in the betterment of the ecosystem:


\paperQuote{Bug-bounty programs offer important security benefits that could be 
useful to many companies. However, our results suggest \hunters 
typically focus on the programs with the most resources (\eg monetary 
rewards, large scopes). Large companies (e.g., Google), 
with committed \bbprograms, are well positioned to take 
advantage in ways smaller companies and programs may not be able to, 
even when these companies are in critical sectors with important security 
needs. Exacerbating the issue, smaller companies are at higher risk for suffering significant loss to cybercrime~\cite{hauman2021smesec, sridhar2021hacking}.}

\paperQuote{Several government agencies currently recommend companies adopt \bbs~\cite{nist2020bugbounties,cisa2020bugbounties}. While this is a good start, without additional support, our results suggest it has the effect of entrenching security inequality.
Government agencies could also provide funding to help companies with lower security budgets and staffing afford to run committed \bbprograms: increasing scope, better staffing, and higher bounties. Grants could be tied to priorities for improving the \bb ecosystem, such as publicizing reports (enabling \hunters to assess programs),  attracting attention to less popular but security-critical industries (e.g., healthcare, finance~\cite{sridhar2021hacking}), or improving existing educational resources~\cite{votipka2021hacked}.}


\paperQuote{Governments have additional roles to play in improving conditions for bug hunters. Legal scholars have proposed legislation to implement legal safe harbors for any good-faith security researcher, including \hunters~\cite{etcovitch2018coming}, and judicial policy-setters have taken steps in this direction~\cite{doj2022goodfaith}. Our work provides evidence that this is a worthwhile effort, as \hunters value a legal safe harbor and use it as a discriminator between programs (\autoref{sec:legal_safe_harbor}). A generalized safe harbor could therefore incentivize \hunter participation for companies that do not currently offer that benefit. %
Further, labor regulators could consider how best to protect \hunters from uncertainty and even abuse associated with gig-work (\autoref{sec:freelance},\cite{ellis2022bounty}), by setting appropriate standards for communication and even payment, which would help to retain more \hunters in the ecosystem.}






\reviewerComment{}{Change as agreed to in the rebuttal.}

\response{We have made the following additional changes:
\begin{itemize}[noitemsep, topsep=0pt]
    \item Minor wording and rephrasing for brevity throughout.
    \item Renaming
``factor-ranking study'' to ``factor-rating study'' to be consistent with the underlying data that we use to determine which factors are most important.
    \item Replaced ``freelance'' with ``gig-work.''
    \item Removed the repetitive conclusion. 
    \item Introduction (\autoref{sec:intro}):
    \begin{itemize}
        \item We slightly rephrased RQ1.
    \end{itemize}
    \item Related Works (\autoref{sec:related})
    \begin{itemize}[noitemsep, topsep=0pt]
        \item Added references to diversity work in vulnerability discovery~\cite{fulton2023v4a} (``Hunters’ self-reported motivation'').
        \item Removed ``\Hunters technical practices'' due to its limited relevance.
    \end{itemize}
    \item Methods (\autoref{sec:method}):
    \begin{itemize}[noitemsep, topsep=0pt]
        \item Clarifying why there are five factor groups listed in 
        Section \ref{subsec:firststudymethods} (we later merged two groups).
        \item Included a brief explanation of why survey participants were not compensated.
        \item Added more details on the logistics of the interviews. 
        \item Noted the estimated overlap between \firststudyps and \secondstudyps (Section~\ref{subsec:ratingmethods}).
        \item Acknowledged that we are unable to account for people who could not find any bugs (early beginners) in Section~\ref{sec:limitations}.
        \item Acknowledged that demographic skews might also skew the bug types and companies that receive attention (Section~\ref{sec:limitations}).
    \end{itemize}
    \item Factors (\autoref{sec:factors}):
    \begin{itemize}[noitemsep, topsep=0pt]
        \item Added references to prior work where necessary. Among other discussions, this includes references to relevant work that found communication to be an issue. We highlight how our results fit into prior observations in Section~\ref{subsec:disputes}.
        \item Added core bug-bounty platform features, as these results were previously excluded for space but are unique to our study (Section~\ref{subsec:platform}). 
        \item Removed ``Other benefits of participating'' to emphasize legal safe harbor details (Section~\ref{sec:legal_safe_harbor}). Later, we refer to these results in the discussion.
        \item Added another quote referencing specific Libraries to better describe \emph{familiarity with technology} (Section~\ref{subsec:learning}).
        \item Clarified that hunters with low and high reputation think reputation plays a role in report acceptance (Section~\ref{sec:finding_bugs}).
    \end{itemize}
    \item Discussion (\autoref{sec:discussion}):
    \begin{itemize}[noitemsep, topsep=0pt]
        \item We added more suggestions on what \bbplatforms can do to address the stress and uncertainty \hunters face. Further, we added recommendations on how governments can fit into this effort.
        \item We clarified that our ideas around insurance policies and increased platform control should be considered in future work.
        \item We acknowledged that some of our recommendations are not cost-free. We suggest that sympathetic governments can play a role in reducing the burden.
        \item We acknowledged increasing scope has nuances and should be explored.
    \end{itemize}
    \item Appendix:
    \begin{itemize}[noitemsep, topsep=0pt]
        \item Removed all sections except additional factors (\autoref{app:additional_factors}) and full list of factors (\autoref{app:full_list}) 
        \item Added the \firststudy survey (\autoref{app:firststudysurvey}) and the \secondstudy survey (\autoref{app:secondstudysurvey}). We present the interview flow in the text (Section~\ref{subsec:interviewmethods})
    \end{itemize}
\end{itemize}
}


